Decentralized Robust Control of Coupled Multi-Agent Systems under Local Signal Temporal Logic Tasks

Motivated by the recent interest in formal methods-based control of multi-agent systems, we adopt a bottom-up approach. Each agent is subject to a local signal temporal logic task that may depend on other agents behavior. These dependencies pose control challenges since some of the tasks may be opposed to each other. We first develop a local continuous feedback control law and identify conditions under which this control law guarantees satisfaction of the local tasks. If these conditions do not hold, we propose to use the developed control law in combination with an online detection & repair scheme, expressed as a local hybrid system. After detection of a critical event, a three-stage procedure is initiated to resolve the problem. The theoretical results are illustrated in simulations.

==> chapter/col_tasks_sec.tex <==

\section{A hybrid system for $\theta$ formulas}
\re{to be rewritten!}The satisfaction of $\theta$ in \eqref{eq:theta1_class} is achieved by a hybrid system $\mathcal{H}=(C,F,D,G)$ with properly defined flow and jump maps $F$ and $G$, and flow and jump sets $C$ and $D$ as discussed in \cite{lindemann2017prescribed}.


Each agent $i$ may be subject to an individual STL formula $\theta$. This formula can include the above mentioned couplings between agents. This means that $\theta$ is a collaborative formula and couplings in the predicates used in $\theta$ will occur. For instance, consider the formula $\theta=\phi=F_{[a,b]}\mu$ with $\rsnt{\mu}=\|\boldsymbol{x}_i-\boldsymbol{x}_j\|\le 5$ imposed on agent $i$. To satisfy this formula, we need that $v_j\in\mathcal{N}_i(t)$ and that $v_j$ does not act as a stubborn agent or have a conflicting formula. Note that $\boldsymbol{x}_j$ can again be seen as an external input to the system.

Tasks that are possible: 
\begin{enumerate}
\item Guarantee/Reachability: $F_{[a,b]} z_1$
\item Progress: $GF_{[a,b]} z_1$ (by looping in hybrid framework)
\item Stability: $F_{[a,b]}G z_1$
\item Response: $G(z_1\implies F_{[a,b]}z_2)$ (hard coded, i.e. in jump map, and used for request\& reply)
\item Sequencing: $F_{[a,b]}(z_1 \wedge F_{[a,b]}(z_2 \wedge \hdots))$
\item Coverage: $F_{[a,b]}z_1 \wedge F_{[a,b]}z_2 \wedge \hdots$
\item Surveillance: $G(F_{[a,b]}z_1 \wedge F_{[a,b]}z_2 \wedge \hdots)$ (looping in hybrid system)
\item Consensus (rather rendezvous): works if agents are connected! (also consensus at predefined locations)
\item Connectivity maintenance by communication leaders $|x_i-x_l|<r$
\item Dispersion of some selected agents
\item Linear/concave (conjunction)/convex(disjunction) predicate cooperative tasks without any restrictions \re{define/explain}
\end{enumerate}

Tasks that might be possible:
\begin{enumerate}
\item Safety: $G_{[a,b]}\neg z_1$ (as a second PPC formula - see next section)
\item Connectivity by each agent (as a second PPC formula - see next section)
\end{enumerate}







%\section{Collaborative tasks}
%\label{sec:col_tasks}
%
%Agents will not only be requested to perform their own individual STL tasks, they will also be subject to collaborative tasks such as consensus, formation control, or just helping another agent perform a task. This is exactly the reason why $\boldsymbol{x}_i^c$ was included in $\rsnt{\psi}$ and which causes the feasibility problems.
%
%\subsection{Consensus}
%Consensus is obtained by imposing the formula
%\begin{align}
%\phi_i=F_{[a,b]}\bigwedge_{j=1}^{\mathcal{N}_i(t)}(|\boldsymbol{x}_i-\boldsymbol{x}_j|<\epsilon)
%\end{align}
%where $\epsilon$ is a small positive constant. Due to connectivity, the agents will eventually within $[a,b]$ agree upon a commonly shared state with precision $\epsilon$.
%
%\subsection{Formation Control}
%Not really possible so far, rather include it into $f_i^c(\boldsymbol{x})$ if there exists a controller for the given dynamics $f_i(\boldsymbol{x}_i)$
%
%\subsection{Connectivity Maintenance}
%
%In multi-agent systems, connectivity maintenance is of high interest. We assume so called communication agents with long-range communication abilities. Consider $M_c$ communication agents, where $M_c<M$. Communication agents can always communicate with other communication agents. Their task is to maintain a maximum distance of $r_c$ to non-communication agents. Hence, each communication agent $j\in\{1,\hdots,M\}$ is subject to the STL formula
%
%\begin{align}
%\phi_i=G_{[0,\infty]}\wedge_{j=1}^{\mathcal{M}_i}(|\boldsymbol{x}_i-\boldsymbol{x}_{j}|\le r_{c})
%\end{align}
%where \re{$\mathcal{M}_i$ needs to be defined properly.}
%
%%Formation control can be obtained in a similar way. We assume pairs of agents $(v_i,v_j)\in E$ that should have a fixed relative distance to each other; denote this set of agents $\mathcal{R}\subset E$. In other words, for an agent $i\in\{1,\hdots,N\}$, there is a set of agents $\Omega_i=\{j\in\{1,\hdots,N\}\setminus j| (v_i,v_j)\in\mathcal{R}\}$ that $i$ needs to have a relative distance to. We impose the formula
%%\begin{align}
%%\phi_i=F_{[a,b]}\bigwedge_{j=1}^{\Omega_i}(|\boldsymbol{x}_i-\boldsymbol{x}_j|\le\epsilon)
%%\end{align}
%%By altering the upper bound in \cite{lindemann2017prescribed}, the distance $|\boldsymbol{x}_i-\boldsymbol{x}_j|$ can be eventually upper and lower bounded.
%


==> chapter/obst_avoid.tex <==
\section{Collision Avoidance}
\label{sec:col_av}


\subsection{Potential Functions}

We could incorporate collision avoidance into the dynamics$f_i^c(\boldsymbol{x})$ by considering potential/navigation functions. However, this is not novel and subject to numerical difficulties while implementing things.

\subsection{Hybrid System}

We can use a hybrid system as a means of communication and event detection scheme.  Next, we define a global critical collision distance $\delta<\min_i r_i$ where $i$ ranges over all possible sensing ranges. Note that $v_iv_j\in E$ means that agent $i$ can send information to agent $j$, not necessarily the other way round.

We can now do event detection, which means basically collision avoidance detection. It basically means that each agent checks if $\vee_{i=1}^{N_i(t)} \|\boldsymbol{x}_i(t)-\boldsymbol{x}_j\|<\delta$. Let us now formulate an initial overall Hybrid systems:


Consider that each agent $i$ is associated with the dynamics
\begin{align}\label{system_noise}
\dot{\boldsymbol{x}}_i&=f_i(\boldsymbol{x}_i)+g_i(\boldsymbol{x}_i)\boldsymbol{u}_i
\end{align}
with $f_i(\boldsymbol{x}_i)\in \mathbb{R}^n$ and $g_i(\boldsymbol{x}_i)\in\mathbb{R}^{n\times m}$. Each agent has its task $\phi_i$ as in \cite{lindemann2017prescribed} and is associated with the hybrid state $\boldsymbol{z}_i=\begin{bmatrix}
q_i & \boldsymbol{x}_i^T & t_i & \Delta_i & \boldsymbol{c}_i^T
\end{bmatrix}$ and the hybrid system $\mathcal{H}_i=\{C_i,F_i,D_i,G_i\}$ where $\boldsymbol{c}_i$ are parameters included in the feedback controller. We extend these systems with a logic for collision avoidance by extending the jump set $C_i$ and jump map $G_i$. Define $\mathcal{C}_{i,col}=\{\boldsymbol{z}_i\in\mathcal{Z}_i| \vee_{i=1}^{N_i(t)} \|\boldsymbol{x}_i-\boldsymbol{x}_j\|<\delta\}$ which detects when agents are in a critical distance. 

The next step after a detection of this event is critical. What do we do in case of a possible collision? Since a collision always has higher priority than the satisfaction of a STL formula $\phi_i$ we should postpone the satisfaction of the formula by risking that we might not be able to satisfy the formula at all (only a relaxed formula). So the idea is twofold:
\begin{itemize}
\item Develop a collision avoidance controller of agent $i$ that does consider the positions of all agents $j\in N_i(t)$ with $\|\boldsymbol{x}_i-\boldsymbol{x}_j\|<\delta$. An idea is to rotate all agents involved in the possible collision in one direction (add a figure here to explain). 
\item Detection of when to turn the collision avoidance controller off and continue with the STL mission. However, the STL task might now be rendered infeasible, therefore a possible formula relaxation needs to be considered as in \cite{ghosh2016diagnosis}. The rough idea is to lower predicates in the formula (hyperplane interpretation in my journal) or to extend the time bounds $[a,b]$ of the formula (might result in timing problems for collaborative tasks). Then, a relaxed formula $\phi$ can be satisfied.
\end{itemize}










==> chapter/sequencing.tex <==
\section{Action Regions}
\label{sec:action_regions}

In multi-agent systems, some regions of interest might be of special interest and might need some special control. 

